GraphFC: Customs Fraud Detection with Label Scarcity

Custom officials across the world encounter huge volumes of transactions. With increased connectivity and globalization, the customs transactions continue to grow every year. Associated with customs transactions is the customs fraud - the intentional manipulation of goods declarations to avoid the taxes and duties. With limited manpower, the custom offices can only undertake manual inspection of a limited number of declarations. This necessitates the need for automating the customs fraud detection by machine learning (ML) techniques. Due the limited manual inspection for labeling the new-incoming declarations, the ML approach should have robust performance subject to the scarcity of labeled data. However, current approaches for customs fraud detection are not well suited and designed for this real-world setting. In this work, we propose $\textbf{GraphFC}$ ($\textbf{Graph}$ neural networks for $\textbf{C}$ustoms $\textbf{F}$raud), a model-agnostic, domain-specific, semi-supervised graph neural network based customs fraud detection algorithm that has strong semi-supervised and inductive capabilities. With upto 252% relative increase in recall over the present state-of-the-art, extensive experimentation on real customs data from customs administrations of three different countries demonstrate that GraphFC consistently outperforms various baselines and the present state-of-art by a large margin.

==> Tables/inspection_rates.tex <==
\begin{table*}[!ht]
\caption{Inspection Rates}
\label{tab:ablation}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{13}{|c|}{\textbf{T-Data}} \\ \hline
Model & Pre.@1 & Rec.@1 & Rev.@1 & Pre.@2 & Rec.@2 & Rev.@2 & Pre.@5 & Rec.@5 & Rev.@5 & Pre.@10 & Rec.@10 & Rev.@10   \\ \hline
GNN\textsubscript{semi}  & 0.829 & 0.087 & 0.143 & 0.737 & 0.156 & 0.248 & \textbf{0.548} & \textbf{0.289} & 0.434 & \textbf{0.376} & \textbf{0.397} & 0.557 \\ \hline
GNN\textsubscript{joint}  & 0.807 & 0.061 & 0.135 & 0.725 & 0.139 & 0.234 & 0.491 & 0.249 & 0.401 & 0.327 & 0.367 & 0.454 \\ \hline
GNN\textsubscript{only} & 0.764 & 0.080 & 0.115 & 0.678 & 0.143 & 0.212 & 0.490 & 0.258 & 0.382 & 0.359 & 0.378 & 0.508 \\ \hline
GNN\textsubscript{sparse} & 0.712 & 0.075 & 0.123 & 0.642 & 0.135 & 0.217 & 0.473 & 0.250 & 0.376 & 0.338 & 0.356 & 0.491 \\ \hline
\model{} & \textbf{0.869} & \textbf{0.092} & \textbf{0.170} & \textbf{0.773} & \textbf{0.163} & \textbf{0.274} & 0.535 & 0.282 & \textbf{0.445} & 0.368 & 0.393 & \textbf{0.557} \\ \hline

\multicolumn{13}{|c|}{\textbf{N-Data}} \\ \hline

GNN\textsubscript{semi}  & 0.281 & 0.113 & 0.162 & 0.251 & 0.203 & \textbf{0.241} & 0.197 & 0.398 & \textbf{0.367} & \textbf{0.135} & \textbf{0.546} & \textbf{0.489} \\ \hline
GNN\textsubscript{joint}  & 0.218 & 0.076 & 0.092 & 0.145 & 0.138 & 0.147 & 0.105 & 0.203 & 0.212 & 0.053 & 0.331 & 0.319 \\ \hline
GNN\textsubscript{only} & 0.068 & 0.027 & 0.069 & 0.053 & 0.043 & 0.107 & 0.034 & 0.069 & 0.157 & 0.027 & 0.109 & 0.243 \\ \hline
GNN\textsubscript{sparse} & 0.067 & 0.070 & 0.120 & 0.059 & 0.125 & 0.203 & 0.044 & 0.234 & 0.359 & 0.032 & 0.346 & 0.483 \\ \hline
\model{} & \textbf{0.401} & \textbf{0.162} & \textbf{0.171} & \textbf{0.332} & \textbf{0.269} & 0.219 & \textbf{0.200} & \textbf{0.405} & 0.304 & 0.129 & 0.524 & 0.411 \\ \hline

\multicolumn{13}{|c|}{\textbf{C-Data}} \\ \hline
GNN\textsubscript{semi}  & 0.030 & 0.024 & 0.034 & 0.023 & 0.037 & 0.056 & 0.023 & 0.092 & 0.127 & 0.022 & \textbf{0.173} & 0.211 \\ \hline
GNN\textsubscript{joint}  & 0.025 & 0.019 & 0.037 & 0.024 & 0.038 & 0.057 & 0.023 & 0.090 & 0.117 & 0.018 & 0.143 & 0.168 \\ \hline
GNN\textsubscript{only} & 0.032 & 0.024 & 0.034 & 0.022 & 0.035 & 0.058 & 0.017 & 0.067 & 0.081 & 0.016 & 0.133 & 0.128 \\ \hline
GNN\textsubscript{sparse} & 0.030 & 0.024 & 0.037 & 0.025 & 0.039 & 0.050 & 0.018 & 0.070 & 0.096 & 0.016 & 0.125 & 0.144 \\ \hline
\model{} & \textbf{0.045} & \textbf{0.035} & \textbf{0.057} & \textbf{0.037} & \textbf{0.058} & \textbf{0.090} & \textbf{0.030} 
& \textbf{0.118} & \textbf{0.170} & \textbf{0.026} & \textbf{0.203} & \textbf{0.267} \\ \hline

\end{tabular}
\end{table*}





==> Tables/ssl-result.tex <==
\begin{table*}[!t]
\caption{Model performance with a 5\% inspection rate. The 5\% ground truth labels are used whereas 95\% of labels are masked.}
\label{tab:ssl-results}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline


\multicolumn{13}{|c|}{\textbf{A-Data}} \\ \hline
Model & Pre.@1 & Rec.@1 & Rev.@1 & Pre.@2 & Rec.@2 & Rev.@2 & Pre.@5 & Rec.@5 & Rev.@5 & Pre.@10 & Rec.@10 & Rev.@10   \\ \hline
XGB  & 0.026 & 0.021 & 0.040 & 0.016 & 0.025 & 0.044 & 0.017 & 0.070 & 0.096 & 0.020 & 0.159 & 0.207 \\ \hline
Tabnet  & 0.031 & 0.024 & 0.031 & 0.021 & 0.033 & 0.032 & 0.016 & 0.061 & 0.049 & 0.014 & 0.109 & 0.083 \\ \hline
DATE  & 0.045 & 0.037 & 0.056 & 0.041 & 0.065 & 0.097 & 0.033 & 0.129 & 0.187 & 0.030 & 0.239 & \textbf{0.358} \\ \hline
$\model{}_{\text{SAGE}}$ & 0.040 & 0.032 & 0.039 & 0.033 & 0.052 & 0.056 & 0.026 & 0.104 & 0.105 & 0.024 & 0.189 & 0.175 \\ \hline
$\model{}_{\text{RGCN}}$ & \textbf{0.050} & \textbf{0.040} & \textbf{0.064} & \textbf{0.044} & \textbf{0.069} & \textbf{0.103} & \textbf{0.039} & \textbf{0.152} & \textbf{0.189} & \textbf{0.033} & \textbf{0.262} & 0.281 \\ \hline
\model{} & 0.045 & 0.035 & 0.057 & 0.037 & 0.058 & 0.090 & 0.030 & 0.118 & 0.170 & 0.026 & 0.203 & 0.267 \\ \hline

\multicolumn{13}{|c|}{\textbf{B-Data}} \\ \hline
XGB  & 0.151 & 0.061 & 0.109 & 0.091 & 0.073 & 0.142 & 0.045 & 0.092 & 0.184 & 0.063 & 0.256 & 0.319 \\ \hline
Tabnet  & 0.149 & 0.060 & 0.089 & 0.087 & 0.071 & 0.126 & 0.046 & 0.085 & 0.171 & 0.047 & 0.189 & 0.291 \\ \hline
DATE  & 0.152 & 0.061 & 0.105 & 0.098 & 0.077 & 0.143 & 0.057 & 0.115 & 0.210 & 0.046 & 0.186 & 0.300 \\ \hline
$\model{}_{\text{SAGE}}$  & 0.327 & 0.132 & 0.143 & 0.285 & 0.231 & 0.208 & \textbf{0.201} & 0.405 & 0.305 & 0.124 & 0.502 & 0.400 \\ \hline
$\model{}_{\text{RGCN}}$  & 0.259 & 0.104 & 0.127 & 0.209 & 0.169 & 0.194 & 0.179 & 0.362 & \textbf{0.334} & \textbf{0.139} & \textbf{0.564} & \textbf{0.458} \\ \hline
\model{} & \textbf{0.401} & \textbf{0.162} & \textbf{0.171} & \textbf{0.332} & \textbf{0.269} & \textbf{0.219} & 0.200 & \textbf{0.405} & 0.304 & 0.129 & 0.524 & 0.411 \\ \hline

\multicolumn{13}{|c|}{\textbf{C-Data}} \\ \hline
XGB  & 0.671 & 0.070 & 0.120 & 0.593 & 0.125 & 0.203 & 0.445 & 0.234 & 0.359 & 0.328 & 0.346 & 0.483 \\ \hline
Tabnet  & 0.715 & 0.050 & 0.081 & 0.651 & 0.137 & 0.223 & 0.452 & 0.231 & 0.334 & 0.331 & 0.349 & 0.469 \\ \hline
DATE  & 0.803 & 0.085 & 0.158 & 0.680 & 0.143 & 0.243 & 0.472 & 0.249 & 0.380 & 0.336 & 0.354 & 0.496 \\ \hline
$\model{}_{\text{SAGE}}$ & 0.788 & 0.083 & 0.135 & 0.722 & 0.152 & 0.242 & 0.535 & 0.282 & 0.442 & 0.371 & 0.392 & \textbf{0.571} \\ \hline
$\model{}_{\text{RGCN}}$  & 0.819 & 0.086 & 0.146 & 0.720 & 0.151 & 0.244 & 0.525 & 0.277 & 0.424 & \textbf{0.373} & 0.393 & 0.556 \\ \hline
\model{} & \textbf{0.869} & \textbf{0.092} & \textbf{0.170} & \textbf{0.773} & \textbf{0.163} & \textbf{0.274} & \textbf{0.535} & \textbf{0.282} & \textbf{0.445} & 0.368 & \textbf{0.393} & 0.557 \\ \hline



\end{tabular}
\end{table*}



 





